Bivariate Semi-Markov Process for Counterparty Credit Risk

We consider the problem of constructing an appropriate multivariate model for the study of the counterparty credit risk in credit rating migration problem. For this financial problem different multivariate Markov chain models were proposed. However the markovian assumption may be inappropriate for the study of the dynamic of credit ratings which typically show non markovian like behaviour. In this paper we develop a semi-Markov approach to the study of the counterparty credit risk by defining a new multivariate semi-Markov chain model. Methods are given for computing the transition probabilities, reliability functions and the price of a risky Credit Default Swap.

==> biblio.tex <==
\bibitem{Barbu}
V. Barbu and N. Limnios, \textsl{Semi-Markov Chains and Hidden Semi-Markov Models Toward Applications: Their Use in Reliability and DNA Analysis}, Ed. Springer (2008).

\bibitem{Bielecki} 
T. R. Bielecki and M. Rutkowski, \textsl{Credit Risk: Modeling, Valuation and Hedging}, Ed. Springer (2004).

\bibitem{Brigo} 
D. Brigo and A. Capponi, \textsl{Bilateral counterparty risk valuation with stochastic dynamical models and application to Credit Default Swaps}, arXiv 0812:3705v4 (2009).

\bibitem{ChingPaper}
W. Ching, E.S. Fung and M.K. Ng, \textsl{A multivariate Markov chain model for categorical data sequences and its applications in demand predictions}, IMA Journal of Management Mathematics, \textbf{13}, 187-199 (2003).

\bibitem{ChKaraLim}
O. Chryssaphinou, M. Karaliopoulou and N. Limnios, \textsl{On Discrete Time Semi-Markov Chains and Applications in Words Occurrences}, Communications in Statistics-Theory and Methods, \textbf{37}, 1306-1322  (2008).

\bibitem{Crepey}
S. Cr\'{e}pey, M. Jeanblanc and B. Zagari, \textsl{Counterparty Risk on a CDS in a Markov Chain Copula Model with Joint Defaults and Stochastic Spreads}, Recent Advances in Financial Engineering World Scientfic (2009).

\bibitem{DamicoManca} 
G. D'Amico, J. Janssen and R. Manca, \textsl{Initial and Final Backward and Forward Discrete Time Non-Homogeneous Semi-Markov Credit Risk Models}, Methodol. Comput. Appl. Prob., \textbf{12}, pag. 215-225 (2010).

\bibitem{DamicoManca2} 
G. D'Amico, J. Janssen and R. Manca, \textsl{A Non-Homogeneous Semi-Markov Reward Model for the Credit Spread Computation}, Int. Journal of Theo. and Appl. Finance, Vol. 14, No. 2, pag. 1-18 (2011).

\bibitem{DamicoManca3} 
G. D'Amico, J. Janssen and R. Manca, \textsl{Valuing Credit Default Swap in a Non-Homogeneous Semi-Markovian Rating Based Model}, Comput. Econ., \textbf{29}, pag. 119-138 (2007).

\bibitem{DamicoManca4} 
G. D'Amico, J. Janssen and R. Manca, \textsl{Discrete Time Non-Homogeneous Semi-Markov Reliability Transition Credit Risk Models
and the Default Distribution Functions}, Comput. Econ., \textbf{38}, pag. 465-481 (2011).

\bibitem{Limnios}
N. Limnios and G. Opri\c san, \textsl{Semi-Markov Process and Reliability}, Ed. Birk\"auser (2001). 

\bibitem{Manca}
J. Janssen and R. Manca, \textsl{Applied Semi-Markov Processes}, Ed. Springer (2006).

\bibitem{Zhu}
M. Pykhtin and S. Zhu, \textsl{Global Association of Risk Professionals}, Issue \textbf{37}, July/August (2007).
